Gravity-aligned Rotation Averaging with Circular Regression

Reconstructing a 3D scene from unordered images is pivotal in computer vision and robotics, with applications spanning crowd-sourced mapping and beyond. While global Structure-from-Motion (SfM) techniques are scalable and fast, they often compromise on accuracy. To address this, we introduce a principled approach that integrates gravity direction into the rotation averaging phase of global pipelines, enhancing camera orientation accuracy and reducing the degrees of freedom. This additional information is commonly available in recent consumer devices, such as smartphones, mixed-reality devices and drones, making the proposed method readily accessible. Rooted in circular regression, our algorithm has similar convergence guarantees as linear regression. It also supports scenarios where only a subset of cameras have known gravity. Additionally, we propose a mechanism to refine error-prone gravity. We achieve state-of-the-art accuracy on four large-scale datasets. Particularly, the proposed method improves upon the SfM baseline by 13 AUC@$1^\circ$ points, on average, while running eight times faster. It also outperforms the standard planar pose graph optimization technique by 23 AUC@$1^\circ$ points. The code is at https://github.com/colmap/glomap.

==> tex/tbl/lamar.tex <==
% \begin{table}[]
%     \centering
%     \resizebox{\columnwidth}{!}{
%     \begin{tabular}{l c c c c c c} \toprule  
%         & AVG ($^\circ$) & MED ($^\circ$) & AUC@$0.5^\circ$ & @$1^\circ$ & @$2^\circ$  & Time (s) \\ \midrule
%         LM 3DoF & 45.18 & 4.80 & \phantom{1}4.18 & 11.42 & 24.33 & 0.58 \\
%         LM 1DoF & 44.51 & 4.12 & \phantom{1}7.86 & 17.55 & 30.49 & \textbf{0.03} \\
%         Theia & \phantom{1}1.09 & 0.70 & 15.25 & 36.65 & 61.44 & 0.09 \\
%         Proposed & \phantom{1}\textbf{0.67} & \textbf{0.35} & \textbf{28.58} & \textbf{53.41} & \textbf{72.43} & \textbf{0.03} \\
%       \bottomrule
%     \end{tabular}
%     }
%     \caption{Average and median rotation errors (in degrees), the AUC score at $0.5^\circ$, $1^\circ$, and $2^\circ$ and average run-time (in seconds) on the LaMAR dataset~\cite{sarlin2022lamar}.}
%     \label{tbl:lamar}
% \end{table}


\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l c c c c c c} \toprule  
        & AVG ($^\circ$) & MED ($^\circ$) & AUC@$0.5^\circ$ & @$1^\circ$ & @$2^\circ$  & Time (hours) \\ \midrule
        LM 3DoF & 45.18 & 4.80 & \phantom{1}4.18 & 11.42 & 24.33 & 1.61 $\times 10^{-4}$  \\ %0.58 \\
        LM 1DoF & 44.51 & 4.12 & \phantom{1}7.86 & 17.55 & 30.49 & \textbf{8.33 $\times 10^{-6}$}  \\ %\textbf{0.03} \\
        Theia & \phantom{1}1.09 & 0.70 & 15.25 & 36.65 & 61.44 & 2.50 $\times 10^{-5}$  \\ % & 0.09 \\
        Proposed & \phantom{1}\textbf{0.67} & \textbf{0.35} & \textbf{28.58} & \textbf{53.41} & \textbf{72.43} & \textbf{8.33 $\times 10^{-6}$}  \\ % \textbf{0.03} \\
        \hdashline
        COLMAP & 10.58 & 0.69 & 21.11 & 33.48 & 43.70 & 7.06 $\times 10^{-2}$ \\
      \bottomrule
    \end{tabular}
    }
    \caption{Average and median rotation errors (in degrees), the AUC score at $0.5^\circ$, $1^\circ$, and $2^\circ$ and average run-time (in hours) on the LaMAR dataset~\cite{sarlin2022lamar}.}
    \label{tbl:lamar}
\end{table}


==> tex/tbl/rebuttal_3dof_E.tex <==
% EuRoC \\
% 1dof \\
% Proposed & \textbf{0.63} & \textbf{0.37} & \textbf{31.17} & \textbf{55.48} & \textbf{73.72} & 7.50 $\times 10^{-5}$ \\
% Theia \cite{theia-manual} & 0.75 & 0.48 & 23.50 & 47.73 & 69.46 & 5.05e+00 \\
% 3dof
% Proposed & \textbf{0.65} & \textbf{0.35} & \textbf{32.68} & \textbf{53.89} & \textbf{72.11} & 5.56 $\times 10^{-5}$ \\
% Theia \cite{theia-manual} & 0.88 & 0.54 & 22.01 & 43.30 & 64.92 & 5.05e+00 \\

% KITTI
% 3dof
% Proposed & \textbf{0.39} & \textbf{0.29} & \textbf{48.71} & \textbf{69.79} & \textbf{83.86} & 5.56 $\times 10^{-5}$ \\
% Theia \cite{theia-manual} & 0.68 & 0.64 & 25.96 & 47.48 & 71.77 & 8.80e+00 \\
% 1dof
% Proposed & \textbf{0.45} & \textbf{0.31} & \textbf{44.49} & \textbf{65.83} & \textbf{81.18} & 8.89 $\times 10^{-5}$ \\
% Theia \cite{theia-manual} & 2.62 & 0.65 & 25.65 & 47.59 & 69.38 & 8.80e+00 \\


\begin{table}[h]
    \centering
    \vspace{-8px}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c l c c c c c c} \toprule 
        &&& AVG ($^\circ$) & MED ($^\circ$) & AUC@$0.5^\circ$ & ~~~~@$1^\circ$~~~~& ~~~~@$2^\circ$~~~~ \\ \midrule
\multirow{4}{*}{\rotatebox{90}{\textit{EuRoC}}} &
\multirow{2}{*}{Proposed} & 5DoF & 0.65 & 0.35 & 32.68 & 53.89 & 72.11 \\
&& 3DoF & \textbf{0.62} & \textbf{0.34} & \textbf{33.94} & \textbf{56.64} & \textbf{74.12} \\
% \hdashline
\cdashline{2-8} 
& \multirow{2}{*}{Theia} & 5DoF & 0.88 & 0.54 & 22.01 & 43.30 & 64.92 \\
&& 3DoF & \textbf{0.77} & \textbf{0.48} & \textbf{23.56} & \textbf{47.05} & \textbf{68.80} \\
\midrule
% \textit{KITTI}\\
\multirow{4}{*}{\rotatebox{90}{\textit{KITTI}}} &
\multirow{2}{*}{Proposed} & 5DoF & \textbf{0.39} & 0.29 & 48.71 & 69.79 & 83.86  \\ 
&& 3DoF & \textbf{0.39} & \textbf{0.27} & \textbf{50.69} & \textbf{70.51} & \textbf{83.98} \\
% \hdashline
\cdashline{2-8} 
&\multirow{2}{*}{Theia} & 5DoF & \textbf{0.68} & 0.64 & 25.96 & 47.48 & 71.77 \\
&& 3DoF & 2.52 & \textbf{0.54} & \textbf{28.79} & \textbf{52.58} & \textbf{72.92} \\
      \bottomrule
    \end{tabular}
    }
    \vspace{-8px}
    \caption{Results with relative poses from both 5-DoF solvers and 3-DoF solvers for EuRoC and KITTI dataset.}
    \label{tbl:rebuttal_3dof_E}
\end{table}
\vspace{-10px}
